Star formation timescale in the molecular filament WB 673

We present observations of ammonia emission lines toward the interstellar filament WB~673 hosting the dense clumps WB~673, WB~668, S233-IR and G173.57+2.43. LTE analysis of the lines allows us to estimate gas kinetic temperature ($\lesssim$ 30~K in all the clumps), number density ($7-17\times10^3$~cm$^{-3}$), and ammonia column density ($\approx 1-1.5\times 10^{15}$~cm$^{-2}$) in the dense clumps. We find signatures of collapse in WB 673 and presence of compact spatially unresolved dense clumps in S233-IR. We reconstruct 1D density and temperature distributions in the clumps and estimate their ages using astrochemical modelling. Considering CO, CS, NH$_3$ and N$_2$H$^+$ molecules (plus HCN and HNC for WB~673), we find a chemical age of $t_{\rm chem}=1-3\times 10^5$~yrs providing the best agreement between the simulated and observed column densities in all the clumps. Therefore, we consider $t_{\rm chem}$ as the chemical age of the entire filament. A long preceding low-density stage of gas accumulation in the astrochemical model would break the agreement between the simulated and observed column densities. We suggest that rapid star formation over a $\sim 10^5$~yrs timescale take place in the filament.

==> all_another_text.tex <==
%The filament is still to be gravitationally unstable as a whole....
%The center of the remnant lies to the west of the filament, the radius of this remnant is 69 $\times$ 54 pc. 
%, its northern part is closer to the center, the southern one is closer to the edge.

{\bf MK stopped here}

%-----------------------------------
%The filament is observed on the periphery of the ionized regions and appears as broken molecular shells on large-scale maps of the CO emission. Young embedded stellar clusters are concentrated in these shells. 
%The formation of five embedded clusters around the \Hii{} region S235 was triggered, or at least accelerated by the expansion of the ionized gas, \cite{2008MNRAS.388..729K, 2014MNRAS.437.1593K, 2016ApJ...819...66D}. Compression, driven by the \Hii{} region S233, could also have impacted nearby star formation \citep{2016AstBu..71..208L}. \cite{2016AstBu..71..208L} find that the prevailing majority of embedded young stellar clusters reside on peripheries of expanding shells in G174+2.5. 
%The distribution of the 13CO column density towards G174+2.5 together with the location of the O-type stars). 
%Our preliminary estimations show that if the possible supernova remnant is on adiabatic (Sedov-Taylor) phase it interacts with the molecular filament.
%-----------------------------------

%Size and mass of the WB~673 filament are in a good agreement with results from the simulations. 
%-----------------------------------

%Ammonia is an important tool for measuring the gas temperature in dense molecular gas \citep[for a review see][]{1983ARA&A..21..239H}. It is still present in the gas phase of very dense (10$^5$ cm$^{-3}$, \cite{2016ApJS..226...13B}) and cold molecular cores \citep{2002ApJ...569..815T}, where the other abundant molecules such as CS and CO are partially frozen into dust particles. 
%Levels of ammonia rotational energy are specified by the total angular momentum $J$ and its projection along the axis of the molecule $K$. Radiative transitions between different $K$~ladders are forbidden, and therefore the lowest meta-stable energy levels are excited only via collisions. Inversion transitions of an ammonia molecule with the same quantum numbers of the upper and lower levels $(J,K)$ are divided into five groups of hyperfine components spaced several MHz. The lowest states in each ladder $(J = K)$ are called meta-stable states, since they can decay only through much slower (10$^{9}$ s) transitions \cite{1983A&A...122..164W}. Therefore, an analytical formulas from the before-mentioned paper obtained in the approximation of local thermodynamic equilibrium (LTE) can be successfully used to analyze the emission intensity of ammonia lines. The ratio of the intensities of the ammonia inversion transitions provides the rotational temperature of the gas, which further can be used to estimate the kinetic temperature. The ratio of hyperfine components provides a measure of optical depth, knowledge of which allows reliable determination of the column density. 
%Our analysis of the ammonia lines follows the work by \citet{1983ARA&A..21..239H}.
%The spectra allow one to obtain the density of a molecular gas according to \cite{1983ARA&A..21..239H}.


\subsection{all other text}

 \cite{2021arXiv210601852Y} suggest that the southern part of the filament WB~673 was formed due to cloud-cloud collision in $\sim$ 0.5 Myr. These estimates agree with our results that the chemical age of clumps is 1 -- 3 $\cdot$ 10$^5$ years.

\cite{2000A&A...361..660P} report that in S233-IR there are 2 different star clusters with ages < 2 and 3 Myr years, and also the age of field stars is 6 Myr years in the S233-IR region, that above our results. The presence of signs of star formation indicates an older age or rapid evolution of molecular clouds.

%Our study showed that clumps WB~668, WB~673, S233-IR and G173.57+2.43 have the similar chemical age of $1-3\times10^5$~years. This indicates the quasi-simultaneous formation of clumps. Cloud formation can be driven by shock waves due supernova remnants or expanding HII regions \citep{2015A&A...580A..49I}. 

%There is the old supernova remnant FVW 172.8+1.5 in the direction of filament WB~673, according to 

%To the west of the filament is a set of regions of ionized hydrogen S231--S233, S235 and several stellar clusters \citep{2017OAst...26...99K}. The age of the supernova remnant much less than the age of  H~II regions, so that it is not possible that the current expanding shell triggered the formation of these HII regions  \citep{2012AJ....143...75K}. The age of supernova remnant FVW 172.8+1.5 similar to found in this work clumps age, so it can influence to formation the dense clumps WB~668, WB~673, S233-IR and G173.57+2.43

%

On the other hand, the simultaneous formation may be due to the dynamic effects of the filament. The gravitational stability of the filament is determined by the mass per unit length. Filaments whose mass per unit length exceeds a critical value collapse along the radius. The critical value depends on the speed of sound, which in turn depends on the temperature.  The total mass of the filament is 10$^4$ M$_\odot$, the mass-to-length ratio M$_{\rm line}$ = 360 M$_\odot$ pc$^{-1}$ from $^{13}$CO (1–0) data, length of the filament from WB~668 in the north-west to G173.57+2.43 in the south-east to be 24.9 pc \cite{2017OAst...26...99K}. According to the formulas from the \cite{2002ApJ...578..914H}, we obtained the values of the critical mass-to-length ratio M$_{\rm line, crit}$ = 54 M$_\odot$ pc$^{-1}$ and  Jeans length $\lambda_c$ = 7 -- 14 pc. So, M$_{\rm line}$ exceeds M$_{\rm line, crit}$ and we see dense clumps in the filament at a distance that is quite close to the Jeans length: the distance between WB~668 and WB~673 is $\sim$ 9 pc, between WB~673 and S233-IR $\sim$ 10 pc, these estimates are given for the assumed distance to the filament D = 1.8 kpc from \cite{1981ApJ...246..394E}. But there is a evolved S233 H~II region between  WB~673 and S233-IR clumps. The distance between the clumps G173.57+2.43 and S233-IR is $\sim$ 3 pc and less than the Jeans length, however, the location of the clump G173.57+2.43 at the end of the filament may be due to the effects of the finite size of the filament, which leads to compaction of the gas at the ends \citep{2016A&A...586A..27K}. On the other side, the H~II region S231 lies near the filament on the east side, so it
can influence to the southern part of the filament, where clumps G173.57+2.43 and S233-IR are located. So, the formation of dense clumps of WB~673 filament could occur under the influence of various triggers: shock wave from supernova remnant FVW 172.8+1.5 in the west of the filament, dynamic effects of the filament itself or H~II region S231 on the east side.






\section*{Appendix 2}

Line (3,3)

\begin{figure*}
	\includegraphics[width=1\linewidth]{map_Tpeak_33_npamax_cut.pdf} 
	\caption{Peak main beam temperature of NH$_3$ (3,3)  line  in the observed clumps. All symbols are the same as in Fig. \ref{fig_int11}.}
	\label{fig_Tpeak33}
\end{figure*}


\section*{Appendix 3}


To study the distribution of line widths and LSR velocities, a Gaussian function was inscribed in the main component of the transition into the emission map of the line (1,1). The distribution of V$_{\rm LSR}$ and $\Delta$V is shown in Fig. \ref{fig_moments}. Velocity gradients are visible in all clumps, in the central clump WB~673 the average speed is lower. The line width is within 1--3.5 \kms and rises closer to the edge of the clumps. In central clumps with more intense radiation, the linewidth is higher than in peripheral.


\begin{figure*}
	\includegraphics[width=1\linewidth]{map_moments.pdf} 
	\caption{LSR velocities (top) and line width (bottom) of NH$_3$ (1,1) main line in WB~668, WB~673, S233-IR and G173.57+2.43. All symbols are the same as in Fig. \ref{fig_int11}.}
	\label{fig_moments}
\end{figure*}


\section*{Appendix 4}

Relations for the search for properties of gravitational stability. 
According to \cite{2019ApJ...877....1D}, virial line mass:
\begin{equation}
M_{line, crit} = \left[1 + \left(\frac{\sigma_{\rm NT}}{c_{\rm s}} \right)^2    \right] \times \left[16~M_\odot pc^{-1} \times \frac{T}{10~K}    \right],
\end{equation}
where $c_{\rm s}$ is sound speed, and $\sigma_{\rm NT}$ is nonthermal velocity dispersion:
\begin{equation}
\sigma_{\rm NT} = \sqrt{\frac{\Delta V^2}{8 \ln{2}} - \frac{k T_{\rm kin}}{30 m_{\rm H}}},
\end{equation}
this $\Delta V$ is observed linewidth of some line with low optical depth, $k$ is Boltzmann constant, $m_{\rm H}$ is proton mass, and thermal velocity dispersion $\sigma_{\rm T}^2 = \sqrt{\frac{k T_{\rm kin}}{30 m_{\rm H}}}$. Sound speed $c_{\rm s}$ must also take into account the dispersion of the gas:
\begin{equation}
c_{\rm s} = \sqrt{c^2 + \sigma_{\rm NT}} = \sqrt{\frac{k T_{\rm kin}}{\mu m_{\rm H}} + \sigma_{\rm NT}},
\end{equation}
where $c$ is thermal sound speed, $\mu$ is mean molecular weight. 
From ammonia median kinetic temperature $T_{\rm kin}$ is 17.2 K,  $\Delta V$ is 3.7 km c$^{-1}$ from C$^{18}$O (1--0) line, which gives thermal sound speed $c$ = 0.25 km~c$^{-1}$, thermal velocity dispersion $\sigma_{\rm T}$ = 0.07 km~c$^{-1}$, nonthermal velocity dispersion $\sigma_{\rm NT}$ = 1.57 km~c$^{-1}$, nonthermal sound speed $c_{\rm s}$ = 1.59 km~c$^{-1}$. The Mach number (i.e. ratio of $\sigma_{\rm NT}$/$c$) = 6.33, which indicating that this regions are supersonic.

According to \cite{2002ApJ...578..914H}, Jeans length  is:
\begin{equation}
\lambda_c = 3.94 \frac{c_{\rm s}^2}{G \Sigma_0},
\end{equation}
where G is gravitational constant, $\Sigma_0$ is surface density, which is defined as the multiplication  of the average radial concentration of hydrogen by the mass of a hydrogen molecule: 
\begin{equation}
\Sigma_0 = 2.016 N(H_2) m_{\rm H}.
\end{equation}
With mean column density $N(H_2) = 1 -- 2 10^{22} cm^{-2}$, $\Sigma_0$ = 0.67 kg m$^{-2}$ and $\lambda_c$ = 7 -- 14 pc.



%\section*{Appendix Anomalies}

%The ratio $=1$ means no anomaly. The ratio for the outer/inner components we designate as HIA$_{\rm OS}$/HIA$_{\rm IS}$, respectively. These values are shown in Fig.~~\ref{fig_hia}. We find the values HIA$_{\rm OS}$ and HIA$_{\rm IS}$ around 1 in all clumps, but also find that some ratio are definitely in particular quadrant in Fig.~\ref{fig_corr_hia}. There is a spatial gradient of the HIA$_{\rm OS}$ and HIA$_{\rm IS}$ values in WB~673: the values $\sim 1.0$ in the northeastern part and $\sim 0.2$ in the southwestern part. HIA$_{\rm OS}$ in clump S233-IR mostly above one, while the values of HIA$_{\rm IS}$ lie near 0.7 and approaches one in the northern part of the clump. We will compare the HIA$_{\rm OS}$ and HIA$_{\rm IS}$ values with results of line emission modelling below.
 

%\textbf{Two models for the hyperfine anomalies}

%There are two models for the formation of a hyperfine structure anomalies of the NH3~(1,1) line. First, the core model, in which the inner satellite from the blue side is enhanced and the outer satellite from the red side due to selective trapping in the far IR (J, K) = (2, 1) $\rightarrow$ (1, 1) transition together with hyperfine selective collisional excitation \citep{1985A&A...144...13S}. The core model assumes that the gas is composed of small individual clumps, those produce ammonia emission with the line widths close to thermal widths. The second model assumes local gradient of velocity due to contraction or expansion of the cloud as a whole. This model predicts that expansion strengthens the inner and outer satellite lines on the red side while suppressing the lines on the other side, and contraction strengthens the lines on the blue side \citep{2001A&A...376..348P, 2004R&QE...47...77T, Pavyar_2008}.

%Fig. \ref{fig_corr_hia} shows the correlation between the values of hyperfine intensity anomalies taking into account the error of definition of the inner and outer satellite for different clumps separately. The dotted lines separate quadrants where the values specific for the two mentioned models should be placed. The values of HIA$_{\rm IS}$ and HIA$_{\rm OS}$ should be placed in the top left quadrant, while the velocity gradient model produces values in the top right and bottom left quadrants.


%It can be seen from Fig.~\ref{fig_corr_hia}, that in our results, taking into account errors, the HIA$_{\rm IS}$ and HIA$_{\rm OS}$ values fall into different quadrants. However, there are some general trends for different clumps. The values of the anomalies in WB~668 are about unity within the error, which may mean the absence of anomalies or contraction. The ratio of the hyperfine satellites in G173.57+2.43 are close to unity within error, however, they tend to the expansion model (HIA$_{\rm IS}$ and HIA$_{\rm OS}$ > 1). HIA$_{\rm IS}$ and HIA$_{\rm OS}$ is enhanced in those directions where the emission is most intense, and in the peripheral clumps of WB~668 and G173/57+2.43 the ammonia emission is not as strong as in the central clumps. It is possible that the values of anomalies around unity in peripheral clumps are explained precisely by the low intensity of ammonia emission.
%A significant part of the values in the WB~673 clump corresponds to the contraction  model with HIA$_{\rm IS}$ < 1 and HIA$_{\rm OS}$ < 1. Most of the values of the S233-IR clump anomalies fall into the upper left quadrant  with HIA$_{\rm IS}$ < 1 and HIA$_{\rm OS}$ > 1, which corresponds to the core model. Some points also fall into the quadrants corresponding to the compression or expansion patterns. We note that the inner satellites are brighter than the outer, therefore, their signal-to-noise ratio is higher and these values are defined with higher precision. It is known, that one of the most studied molecular outflow is located in the S233~IR clump~\citep[e.~g.][]{2002A&A...387..931B, 2007A&A...466.1065B}.




%%%%%%%%%


%\begin{itemize}
    %\item Maps of the integrated intensity of the NH$_3$ (1,1) and (2,2) lines in the dense clumps show that bright ammonia emission correlates with the dust continuum emission. An analysis of the emission lines of ammonia  NH$_3$ (1,1), (2,2) and (3,3) in the peaks of the integral intensity of the transition (1,1) was carried out. 
    
    %\item The distribution of the optical depth of ammonia in the transition (1,1) is obtained. The NH$_3$~(1,1) lines are moderately thick with $\tau_{\rm (1,1)} \leq 2$. The optical depth increases in the densest central parts of the clumps.
    
    %\item The distribution of the ammonia column density, the kinetic temperature of the gas and the abundance of ammonia in relation to hydrogen is obtained. The peak of the column density has a shift to the north-east relative to the dust emission peak at 1.1~mm in the central clump WB~673, however, it correlates well with the 22~micron emission. The gas kinetic temperature increases in the direction of the densest central parts of the clumps, while the abundance of ammonia decreases in this direction.
    
    %\item An analysis of the anomalies of the hyperfine structure of ammonia lines in the (1,1) transition is carried out. It is shown that the values of the anomalies in the central clump WB~673 correspond to the contraction model, and the clump S233-IR corresponds to the core model.
%\end{itemize}



